Private, Efficient, and Accurate: Protecting Models Trained by Multi-party Learning with Differential Privacy

Secure multi-party computation-based machine learning, referred to as MPL, has become an important technology to utilize data from multiple parties with privacy preservation. While MPL provides rigorous security guarantees for the computation process, the models trained by MPL are still vulnerable to attacks that solely depend on access to the models. Differential privacy could help to defend against such attacks. However, the accuracy loss brought by differential privacy and the huge communication overhead of secure multi-party computation protocols make it highly challenging to balance the 3-way trade-off between privacy, efficiency, and accuracy. In this paper, we are motivated to resolve the above issue by proposing a solution, referred to as PEA (Private, Efficient, Accurate), which consists of a secure DPSGD protocol and two optimization methods. First, we propose a secure DPSGD protocol to enforce DPSGD in secret sharing-based MPL frameworks. Second, to reduce the accuracy loss led by differential privacy noise and the huge communication overhead of MPL, we propose two optimization methods for the training process of MPL: (1) the data-independent feature extraction method, which aims to simplify the trained model structure; (2) the local data-based global model initialization method, which aims to speed up the convergence of the model training. We implement PEA in two open-source MPL frameworks: TF-Encrypted and Queqiao. The experimental results on various datasets demonstrate the efficiency and effectiveness of PEA. E.g. when ${\epsilon}$ = 2, we can train a differentially private classification model with an accuracy of 88% for CIFAR-10 within 7 minutes under the LAN setting. This result significantly outperforms the one from CryptGPU, one SOTA MPL framework: it costs more than 16 hours to train a non-private deep neural network model on CIFAR-10 with the same accuracy.

==> tex/0.response.tex <==
\twocolumn[
\begin{center}
    {\Large  \bf Revision Summary}
\end{center}

We sincerely thank all the reviewers for their insightful comments. In this file, we provide a combined PDF following the instructions documented in the notification email. We first provide a summary of changes that we have made in the revised paper according to the comments. Next, we detailedly explain how we address the other issues raised in the individual reviews. Subsequently, we show the revised version of our paper. Lastly, we show a version of the paper with all the major changes highlighted in blue color.


We first respond point by point to the list of expectations provided with the revise decision as follows.

% We have carefully  revised the paper a
% thoroughly as follows: (1) For statements that require further justification (mentioned by Reviewer A, Reviewer B, and Reviewer C), we justify all of them to show the correctness of our method. (2) For extra experiments mentioned by Reviewer A, we conduct them for ablation study to further show the effectiveness of our method. (3) For previous studies mentioned by Review A, Reviewer B, and Reviewer C, we compare our method with these studies to further show the novelty and advantages of our method. (4) For unclear expressions and the problematic claim mentioned by Reviewer A and Reviewer D,  we correct the expressions and remove the claim to avoid misunderstanding. (5) For missing details mentioned by Reviewer D, we supplement the details of protocols to help readers understand our method. (6) We thoroughly polish the expression of our paper.
\vspace{0.05in}    
   (1) \textbf{justify why the data-independent feature extraction does not need to be analyzed within the DP framework.}
    
\vspace{0.05in}    
    \textbf{Response:} In Section~\ref{subsec:separate}, we explain why the data-independent feature extraction does not need to be analyzed within the DP framework. We show them as follows:
    
    \begin{quote}\textcolor{blue}{Because we perform the global model training process on secret shared data, the extracted features are invisible to potential adversaries (i.e. other parties, the users of trained models). Meanwhile, as we utilize secure DPSGD to protect the trained model, the feature extraction operation is oblivious to the adversaries.  In other words, the data-independent feature extractor can be viewed as the ``frozen part'' of a large pre-trained model, and the trained shallow model can be viewed as the ``tuned part'' of the model. The ``frozen part'' does not need to be protected by DP as it is not tuned. This conclusion is the same as those of previous studies~\cite{yu2022differentially, tramer2021differentially}.}
    \end{quote}
 
    \vspace{0.05in}  
      (2) \textbf{fix Lemma 2 issue mentioned by reviewer A.}
    
    \vspace{0.05in}  
    \textbf{Response:}  We fix the expression issue of Lemma~\ref{lemma:error_bound}, where we change the `$x$' as `$x'$' to avoid misunderstanding. Furthermore, in Section~\ref{Sec:Inverse}, we show that Lemma~\ref{lemma:error_bound} implies the DP guarantee of true gradient vectors. We show that, according to Lemma~\ref{lemma:error_bound}, we can guarantee that the $L_2$ norms of clipped gradient vectors are smaller than $C$. As a result, we can obtain the DP guarantee of true gradient vectors.
 
\vspace{0.1in}    
   (3) \textbf{justify how the SMC protocol ensures that minibatches are sampled randomly and randomness is kept secret (to ensure privacy amplification results still hold).}
    
    \vspace{0.05in}  
    \textbf{Response:}  In Section~\ref{subsec:secure_DPSGD}, we show that SMPC protocols can ensure that minibatches are sampled randomly and keep the randomness secret for parties. We show our analysis as follows:
    \begin{quote}
    \textcolor{blue}{Protocol~\ref{alg:secure_dp_sgd} amplifies the privacy guarantee of the training process by randomly sampling minibatches from the logically global dataset. We apply the recently proposed oblivious shuffling protocols~\cite{chida2019efficient, movahedi2015secure, laur2011round}, each of which can securely shuffle the logically global dataset while keeping the new permutation of data samples invisible to parties, to implement the random sample operation. With these oblivious shuffling protocols, we can securely sample minibatches to meet the requirement of DPSGD.}
    \end{quote}

 
  
\vspace{0.05in}    
    (4) \textbf{adding accuracy comparison w/ and w/o MPC for ablation study.}
    
    \vspace{0.05in}  
    \textbf{Response:}  In Section~\ref{subsec:effectiveness_MPL}, we add accuracy comparison w/ and w/o SMPC for ablation study. The experimental results show that SMPC has a negligible impact on the accuracy of the trained models. The main reason is that we apply SMPC protocols to simulate a trusted server that could virtually hold all data from parties to train the target model~\cite{lindell2017simulate}. We further discuss the reasons for the impact brought by SMPC in Section~\ref{subsec:effectiveness_MPL} as follows:
    \begin{quote}
        \textcolor{blue}{The possible impact of SMPC mainly comes from two factors: (1) we perform the computation over fixed-point numbers. However, they can only express the decimal number with limited precision, which might bring a negligible accuracy loss to the trained models. (2) we use linear piecewise functions to approximate non-linear activation functions (e.g. sigmoid function), which would bring another negligible accuracy loss.}
    \end{quote}
 
   \vspace{0.05in}  
(5) \textbf{comparison with papers on federated learning and secure aggregation with DP is missing (add at least a comparison with [a] and [b] from review A, Chase et al. and \texttt{CrypTen} from review B).}
    
\vspace{0.05in}  
\textbf{Response:}  In Section~\ref{subsec:FL_secure_DP}, we empirically compare our proposed secure DPSGD protocol and its optimized implementations with both CAPC Learning~\cite{choquette-choo2021capc} and Distributed Discrete Gaussian~\cite{kairouz2021distributed} mentioned by Reviewer A, which are two state-of-the-art methods on federated learning and secure aggregation with DP. The results show that the models trained by our proposed secure DPSGD protocol and its optimized implementations are more accurate than models trained by CAPC Learning and Distributed Discrete Gaussian. For example, when evaluated on the CIFAR-10 dataset, the accuracy of models trained by \tfencrypted and \queqiao is about 88.99\% and 88.18\% respectively. In contrast, the accuracy of models trained by CAPC Learning and Distributed Discrete Gaussian is 57.31\% and 41.57\% respectively.
    
  
 ]
\twocolumn[ 
 \quad\quad We further compare our proposed secure DPSGD protocol with previous studies mentioned by  Reviewers A and B in Section~\ref{related_work} as follows.
 
\begin{quote}
    \textcolor{blue}{ They apply SMPC protocols to securely aggregate the intermediate information (i.e. noisy gradient vectors or noisy labels) of the training process, which implies relatively higher efficiency and scalability.  However, transferring intermediate information inevitably causes considerable accuracy loss to trained models~\cite{yang2019federated}, especially when the data are not independent and identically distributed among parties~\cite{yang2019federated}. As a result, when the number of parties is small, our proposed secure DPSGD protocol is more suitable than these methods.}
\end{quote}

\quad\quad Note that \texttt{CrypTen} is an MPL framework rather than a federated learning framework. Thus, we separately compare our proposed secure DPSGD protocol with it in Section~\ref{subsec:e_a_inverse}.


\vspace{0.1in}
(6) \textbf{comparison of the data-independent feature extraction to Tramer and Boneh.}
    
    \vspace{0.05in}  
    \textbf{Response:}  In Section~\ref{related_work}, we compare our proposed data-independent feature extraction method with previous studies on the utility optimization of DPSGD~\cite{papernot2020making,zhou2021bypassing,dimension_reduction,tramer2021differentially}, including the method proposed by Tramèr and Boneh.  We show that these studies mainly focus on the centralized setting and only aim to reduce the accuracy loss brought by DPSGD. In particular, Tramèr and Boneh only consider the image classification task. Different from these previous studies, we are the first to consider the data-independent feature extraction for general tasks in the distributed setting. Furthermore, we identify that the method can significantly improve the efficiency of the training process of MPL.
    
    \vspace{0.1in}  
    (7) \textbf{remove claims of model inversion defense. }
    
    \vspace{0.05in}  
    \textbf{Response:}  After carefully investigating previous results, we remove the claim that DPSGD can defend against the model inversion attacks in the revised paper.

\vspace{0.1in}
    (8) \textbf{add missing details for the protocol per review D.}
    
    \vspace{0.05in}  
    \textbf{Response:} We supplement the missing details of protocols according to comments from Reviewer D. Firstly, we clarify the points that might lead to misunderstanding, including the usage of feature extractors (Section~\ref{subsec:summary}), the secure selection of a random minibatch (Section~\ref{subsec:secure_DPSGD}), the phase of decryption (Section~\ref{subsec:secure_DPSGD}), and the equality of each participant (Section~\ref{pre:smpc}). Meanwhile, we correct the expression issue of Line 2 of Protocol~\ref{alg:secure_dp_sgd} (i.e. using the global model initialized by Protocol~\ref{alg:global_model_initialization} rather than the randomly initialized model). Finally, we supplement the details of  ``secret sharing and reconstruction'' (``encryption and decryption'' mentioned by Reviewer D) in Section~\ref{pre:smpc}.
    
\vspace{0.2in}

    \begin{center}
    {\Large  \bf Detailed Response}
\end{center}
We then explain how we address the other issues raised in the individual reviews from reviewers as follows.
    
    \begin{center}
    {\large  \bf To Reviewer \#116A}
\end{center}

\textbf{Comment:} {\it It is interesting to see low accuracy effect of DP. What if one were to use the same methods without MPC; would this improve performance of DPSGD as well (for example, comparing it against LENET/SampleNet and floating points). In general, please consider adding accuracy comparison w/ and w/o MPC for ablation study.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In Section~\ref{subsec:effectiveness_MPL}, we compare the accuracy of models trained by MPL on the logically global dataset and the accuracy of models centrally trained on the global dataset in the plaintext form for the ablation study. The results show that SMPC only has a negligible impact on the accuracy of trained models. We also discuss the potential reasons for the impact in Section~\ref{subsec:effectiveness_MPL}.

\vspace{0.1in}
\textbf{Comment:} \textit{How does the method compare with: (a). CaPC Learning: Confidential and Private Collaborative Learning. ICLR 2021. Choquette-Choo et al. (b). The Distributed Discrete Gaussian Mechanism for Federated Learning with Secure Aggregation. ICML 2021. Kairouz et al.}


    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We first empirically compare our proposed secure DPSGD protocol and its optimized implementations with Paper (a) and Paper (b) mentioned by you in Section~\ref{subsec:FL_secure_DP}. The results show that the models trained by \tfencrypted and \queqiao are more accurate than models trained by these two methods. We further discuss the differences between our proposed secure DPSGD protocol and the methods you mentioned in Section~\ref{related_work}.





 ]
\twocolumn[ 
\textbf{Comment:}\textit{ Please give more details on data-independent feature extraction as it is not immediately clear why this does not have to be done with DP protection.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We detailedly explain why data-independent feature extraction does not need to be done with DP protection in Section~\ref{subsec:separate}.

\vspace{0.1in}
\textbf{Comment:} \textit{In Noise generation ``Byzantine robustness'' was mentioned. This however seems to be a property only of this subprotocol, it is worth pointing out that this is (or may be not) the property of the end-to-end protocol.}


    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We clarify that Byzantine robustness is only the property of the noise generation subprotocol instead the end-to-end secure DPSGD protocol in Section~\ref{Sec:Noise_Gen}.
\vspace{0.1in}



\textbf{Comment:} \textit{DP guarantees of [49]. The statement on [49] was a bit confusing. If the approximate value is higher than C, would not it be clipped in Line6 of Alg 1 as it is the approximate value that is clipped?}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In Section~\ref{Sec:Inverse}, we further clarify the statement on the previous study on secure inverse of square root. When the approximated $L_2$ norm of one gradient vector is smaller than or equal to $C$ (i.e. $\frac{C}{\left\| \nabla\ell(\theta;s_i) \right\|_2^{\mathit{approx}}} \geq 1$), the gradient vectors will not be clipped. 

\vspace{0.1in}
\textbf{Comment:} \textit{Lemma 2 shows the approximate value will always be smaller than the real value. Please add this to show that using a smaller approximate value + noise guarantees DP of the true value. Also, I may have missed why x is in [0.5,1) for DPSGD.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We modify the `$x$' in Lemma~\ref{lemma:error_bound} as `$x'$' to avoid misunderstanding. Furthermore, we show how Lemma~\ref{lemma:error_bound} implies the DP guarantee of Protocol~\ref{alg:secure_dp_sgd} in the last paragraph of Section~\ref{Sec:Inverse}.

\vspace{0.1in}

\textbf{Comment:}\textit{ Please elaborate on 3 party limitation of TF-Encrypted.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In the caption of Table~\ref{tab:effectiveness_MPL_CIFAR}, we state that \texttt{TF-Encrypted} can only support the scenarios with three training parties because its back-end SMPC protocol (i.e. \texttt{ABY3}) only supports the 3-party scenario.

\vspace{0.1in}
    \begin{center}
    {\large  \bf To Reviewer \#116B}
\end{center}


\textbf{Comment:} \textit{The paper's first stated contribution is an MPC protocol for DPSGD. However, there are other works that proposed MPC protocols for DPSGD (e.g. ``Private Collaborative Neural Network Learning'' by Chase, Gilad-Bachrach, Laine, Lauter, and Rindal). These aren't mentioned or compared against, so it's hard to evaluate this paper's contribution.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In Section~\ref{related_work}, we show the differences between our proposed secure DPSGD protocol and the method you mentioned. Our proposed secure DPSGD protocol is designed for SMPC-based machine learning frameworks and wholly implemented by SMPC protocols. Therefore, our proposed secure DPSGD protocol is different from the FL-based method you mentioned, which only uses SMPC protocols to aggregate the intermediate information of the training process. 


\vspace{0.1in}
\textbf{Comment:} \textit{Similarly, the paper designs a secure inverse square root protocol but doesn't compare to other works that do to the same. \texttt{CrypTen} is mentioned as not having a direct computation of inverse square root but rather separate square root and reciprocal functions; combining these seems like a perfectly valid way of computing inverse square root though, so it is not clear what weaknesses of previous protocols for this functionality the proposed construction is improving on.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In the first paragraph of Section~\ref{Sec:Inverse}, we discuss one previous method~\cite{inverse_root_ccs} that uses polynomial to directly approximate the inverse square root. We show that the method has two issues: (1) it is based on the mixed protocols (e.g. \texttt{ABY3}), while ours is based on linear secret sharing protocols and can be applied to more MPL frameworks. (2) the error of its polynomial approximation might destroy the privacy guarantee of DPSGD, while we avoid destroying the privacy guarantee by proving the upper bound of the approximation error. Therefore, our proposed secure inverse square root protocol is highly non-trivial compared with the previous study. As to \texttt{CrypTen}, it has relatively lower efficiency than our proposed secure inverse square root protocol. More importantly, \texttt{CrypTen} is accurate only for those input values in a fixed range (e.g. [0.1, 200)). The main reason is that it uses the Newton-Raphson method to approximate the target function. Thus its approximation errors are highly dependent on the pre-defined initial point and iteration number.  We show the corresponding results and descriptions in Section~\ref{subsec:e_a_inverse} of the revised paper.


]
\twocolumn[ 


\textbf{Comment:} \textit{Given the above, I feel that the contribution of the paper is mostly on the ML side rather than the security/privacy side, which may not be good a fit for S\&P.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We argue that our study is definitely a good fit for IEEE S\&P because we are the first to enhance the privacy protection of existing secret sharing-based MPL frameworks by integrating DPSGD into these frameworks.
Actually, our proposed secure DPSGD protocol solves a very important privacy issue of existing MPL frameworks, many of which~\cite{mohassel2018aby3,DBLP:conf/sp/MohasselZ17,cryptGPU,fantastic-four} are published in top security/privacy conferences.

\vspace{0.1in}
\textbf{Comment:} \textit{I'm also wondering whether the datasets and tasks chosen were complex enough that these results would generalize to other uses of neural networks.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.  We choose to evaluate image classification and sentiment analysis because these two tasks are classical tasks in the artificial intelligence field and are also widely evaluated by previous studies on privacy-preserving machine learning~\cite{mohassel2018aby3,cryptGPU,DBLP:conf/sp/MohasselZ17,Bu2020Deep}. Meanwhile, the datasets that we evaluated are also widely used in previous studies~\cite{cryptGPU,DBLP:conf/sp/MohasselZ17,Bu2020Deep}. Moreover, the generality of foundation models has been proven by literature~\cite{foundation_model,jumper2021highly, rothchild2021c5t5,chen2021decision}.

\vspace{0.1in}
\textbf{Comment:} \textit{``Encryption'' should not be used interchangeably with ``secret sharing'', as they are different cryptographic primitives and the paper should be precise when it comes to security and privacy}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. To keep the preciseness and consistency of our expression, we replace all ``Encryption'' and ``Decryption'' in our paper with ``Secret sharing'' and ``Reconstruction'', respectively.

\vspace{0.1in}
\textbf{Comment:} \textit{Section IV.A - protocol steps are written as if each party $P_i$ does each step locally instead of on shares under MPC}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We argue that the descriptions of our protocols clearly show that they are performed on shares. In Table~\ref{tab:notations}, we show that we use angle brackets to mark shares. In the following four protocols involved in our paper, we show the computations on shares by adding angle brackets to mark shares held by different parties.

\vspace{0.1in}
\textbf{Comment:} \textit{Only online complexity is listed - offline complexity should be listed as well even if it can be precomputed}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We supplement the offline complexity of Protocol~\ref{alg:secure_inversesqrt} and Protocol~\ref{alg:secure_dp_sgd} Appendix~\ref{sec:analysis_inversesquareroot}, Appendix~\ref{sec:analysis_secure_dpsgd} respectively. For other protocols, as they do not have the offline phase, we do not analyze their offline complexity.

\vspace{0.1in}
\textbf{Comment:} \textit{Protocol 3, line 4 - $P_i$ samples B from D. Don't all parties need to sample the same subset of D? How is this done?}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. Yes, different parties sample the same subset. This can be achieved by running oblivious shuffling protocols. We discuss this point in detail in Section~\ref{subsec:secure_DPSGD}.

\vspace{0.1in}
\textbf{Comment:}\textit{ Protocol 3, line 5 - what is the complexity of computing the gradient under MPC?}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. This complexity depends on the concrete secret sharing protocols and types of trained models. For example, to compute one gradient vector for the logisitc regression model, \texttt{ABY3}~\cite{mohassel2018aby3} (the back-end protocol of \texttt{TF-Encrypted}) requires $\log k+3$ communication rounds and $23k+2pk$ bits of communication, while \texttt{Queqiao}, which is a MPL framework based on the BGW protocol~\cite{ref_gmw}, requires 6 communication rounds and $2k^2+2pk+6k$ bits of communication, where $k$ is the number of bits to represent data, and $p$ is the dimension of the gradient vectors. 

% We refer more details about the complexity of gradients computation to previous studies~\cite{mohassel2018aby3,DBLP:conf/sp/MohasselZ17,wagh2020falcon} on MPL.

% Our goal is to design a secure DPSGD protocol based on general linear secret sharing schemes. We refer the complexity of gradients computation to previous studies~\cite{mohassel2018aby3,DBLP:conf/sp/MohasselZ17,wagh2020falcon} on MPL.

\vspace{0.1in}
\textbf{Comment:} \textit{p. 7 says training models based on foundation models has rapidly emerged as a new paradigm but only gives one citation - can you give more examples and say more about this?}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In Section~\ref{subsec:separate}, we supplement more citations to support our statement about the popularity of foundation models.

\vspace{0.1in}
\textbf{Comment:} \textit{Choosing most accurate local model - how is this done and on what data? If it is done under MPC this would be expensive.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We show the pseudocodes of choosing the most accurate local model in Protocol~\ref{alg:maximum_aggregation} of  Appendix~\ref{sec:secrity_complexity_analysis}. The operation is done on the testing data that was generated by first obliviously shuffling the logically global dataset and then partitioning it to training data and testing data. It could not be expensive as it only requires parties to perform secure inference on a few testing data $m$ times, where $m$ is the number of parties.

\vspace{0.1in}
\textbf{Comment:} \textit{p. 8 ``arbitrarily more than three parties'' - should this be ``more than two parties''?}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We correct our expressions in Section~\ref{subsec:experiment_setup} to avoid misunderstanding.

 ]
 
\twocolumn[


\textbf{Comment:} \textit{p. 7 ``As these candidate models are protected by differential privacy and testing data are not visible to parties, the accuracy does not leak private information'' - This doesn't seem necessarily true, since DP does not mean no information is revealed at all.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We argue that the intermediate accuracy would not expose private information about the training dataset as the testing dataset is invisible to parties. The inference of testing data is performed on secret-shared data rather than plaintext data. Therefore, parties have no information about testing data and cannot infer the information of trained local models from the intermediate accuracy. 



\vspace{0.1in}
\textbf{Comment:} \textit{Field sizes in Queqiao and TF-Encrypted implementations are rather different; what is the reason for not using more similar field sizes?}



    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We state the reason for the different field sizes in Section~\ref{subsec:experiment_setup}. The difference of field sizes in \texttt{Queqiao} and \texttt{TF-Encrypted} is originated from their different back-end protocols. \texttt{Queqiao} is based on the BGW protocol, which performs secure computation over the prime field. In contrast, \texttt{TF-Encrypted} is based on the \texttt{ABY3} protocol, which performs secure computation over the integer ring.

\vspace{0.1in}
\textbf{Comment:} \textit{Figure 2 performance graphs look unnecessarily complicated with the zoom-in boxes and many curves}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We modify the performance graphs of Figure~\ref{fig:e2e_comparision} to avoid unnecessary complications.

\vspace{0.1in}
\textbf{Comment:} \textit{Figure 3 - interpret what is happening for the highest input values}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.  We supplement the interpretation of this point in Section~\ref{subsec:e_a_inverse}. \texttt{CrypTen} can only be accurate for input values in [0.1, 200) as it uses the Newton-Raphson method to approximate the target function iteratively. Its approximation errors are highly dependent on the pre-defined initial point and the iteration number. Therefore, \texttt{CrypTen} could be accurate for those input values in a fixed range while having a large error for other input values.
 
 \vspace{0.1in}
\textbf{Comment:} \textit{Table IV - ``locally trained'' vs. ``globally trained'' models makes it sounds like it's about where the training happens, but the important difference is whether it's a subset or the full dataset}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We modify the caption of Table~\ref{tab:effectiveness_MPL_CIFAR} (Table IV of our original submission) to avoid misunderstanding.

\vspace{0.1in}
\textbf{Comment:} \textit{I wasn't convinced by the claim that backdoor attacks are not a risk in this setting. More details would be helpful.}

    \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. In Section~\ref{subsec:backdoor_attacks}, we state that two backdoor attacks~\cite{jia2022badencoder,9581257} on foundation models instead all backdoor attacks would cause little privacy risk to MPL. The reason is that backdoor attacks on foundation models assume that adversaries hold some training data for downstream tasks. With the strict protection of highly sensitive training data  (e.g. medical images) in the context of MPL, attackers would be difficult to obtain these data samples, thus leading to little privacy risk to the trained models. Besides, to further defend the backdoor attacks on foundation models, the owners of trained models can employ recently proposed defenses (e.g. MNTD~\cite{xu2021detecting}) to detect the backdoors hidden in the trained models.

\vspace{0.1in}
\textbf{Comment:} \textit{The paper says future work will integrate recent optimizations on DPSGD. Which ones? More details would be helpful.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We supplement the details of recent optimizations on DPSGD in Section~\ref{subsec:future_work}.

\vspace{0.1in}
    \begin{center}
    {\large  \bf To Reviewer \#116C}
\end{center}

\textbf{Comment:} \textit{The citation to DP-SGD is wrong. It is not Abadi et al. It was first introduced in Song et al. 2013, formally analyzed in Bassily et al. 2014, improved by Abadi et al. 2015 via moments accountant.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. We correct the citation to DPSGD by adding the citation to Song et al. 2013 at places we cite DPSGD.

\vspace{0.1in}
\textbf{Comment:} \textit{One of the main applicability of DP-SGD relies on either privacy amplification by sampling/shuffling. I was not clear on how the SMC protocol ensures this. The privacy guarantee of DP-SGD relies on keeping the randomness in the sampling process secret. So, the SMC protocol needs to take care of it.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.  We show that the privacy amplification of our proposed secure DPSGD protocol can be achieved by running oblivious shuffling protocols. We discuss this point in detail in Section~\ref{subsec:secure_DPSGD}.




% \textbf{Comment:} Typos.

% \textbf{Response:} Thanks for the insightful comment. We thoroughly polish the expression of our paper to eliminate typos and grammatical mistakes.

]

\twocolumn[


\textbf{Comment:} \textit{The optimization methods mentioned in the paper (both feature extraction, and model initialization) seem tangential to the core problem.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment. The optimization methods are highly relevant to resolve our problem, i.e. how to securely and efficiently train an accurate differentially private machine learning model over the distributed data among parties. As we discussed in Section~\ref{intro}, while we can apply SMPC protocols and DPSGD to securely utilize private data from different parties, efficiency and accuracy become two main obstacles to applying these two techniques in practice. Our first optimization method optimizes both efficiency and accuracy of differentially private multi-party learning. The second optimization method accelerates the convergence of the training process. Therefore, our optimization methods can significantly improve the efficiency and accuracy of differentially private multi-party learning and help to resolve our core problem. Furthermore, our proposed optimization methods are also applicable in other systems (e.g. federated learning-based systems).

\vspace{0.1in}
\textbf{Comment:} \textit{ Furthermore, there are existing results which propose these ideas (e.g. Tremmer and Boneh).}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.   The local data-based model initialization method is totally different from the method proposed by Tramèr and Boneh. As to the data-independent feature extraction method, we compare our proposed method with the method proposed by Tramèr and Boneh in Section~\ref{related_work}. We show that compared with previous studies on the utility optimization of DPSGD, we are the first to consider the data-independent feature extraction method in the distributed setting for general tasks. Furthermore, we identify the specific advantage on the efficiency of the method in the distributed setting.

\vspace{0.1in}
    \begin{center}
    {\large  \bf To Reviewer \#116D}
\end{center}

\textbf{Comment:} \textit{ DPSGD does not protect against inversion attack, as it is mentioned in the paper many times. Indeed, the inversion attack reconstruct some data points which are representative of a group, while the DPSGD only protect individual records. Therefore, to protect against this attack, the Client-Level DP protection should be considered.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.  After carefully investigating previous studies, we remove the claim that DPSGD can defend against the model inversion attacks in the revised version of our paper. Moreover, we put implementing the defenses against model inversion attacks in MPL frameworks as our future work in Section~\ref{subsec:future_work}.


\vspace{0.1in}
\textbf{Comment:} \textit{Some details are needed in the paper:}

\textit{2-a)-The feature extractor is used only during the local training of the shallow models, or the secret shared data also are based on extracted features? }

\textit{2-b) Protocol 3, line 2, at this step, the initialized global model should be used instead of using random initialized model.}

\textit{2-c) Protocol 3, line 4, a random batch is selected from the local dataset or the logically global dataset? The latter should be more described. }

\textit{2-d) Protocol 3, after line 17, the averaged encrypted global model is decrypted collaboratively over the m clients before starting the round t+1?}

\textit{3-e) It is not clear at which step the decryption is performed? Is it at the end of the training or after each round?}

\textit{4-f) You do not have a server as it is the case in standard Federated Learning, but you have this notion of global model and logical global dataset, does it mean that you are considering each participant as a server for all the other participants (purely decentralized learning)? }

\textit{4-g) The subsection “Encryption and Decryption” needs to be more detailed.}

 \vspace{0.05in}  
\textbf{Response:} Thanks for the insightful comment.  We supplement the details of protocols according to the comments as follows.

\noindent2-a), in Section~\ref{subsec:summary}, we clarify the phase of using the feature extractor as follows:

\begin{quote}
    
\textcolor{blue}{Note that this step is completed locally. And the following training processes are performed on the extracted features.}
\end{quote}
\noindent2-b), in Line 2 of Protocol~\ref{alg:secure_dp_sgd}, we change the global model initialization method as follows:

\begin{quote}
\noindent\textcolor{blue}{Initializing $\share{\theta_1}_i$ with Protocol~\ref{alg:global_model_initialization}}.
\end{quote}
\noindent2-c), in Section~\ref{subsec:secure_DPSGD}, we show how SMPC protocols sample a random batch from the logically global dataset as follows:

\begin{quote}
\noindent\textcolor{blue}{Protocol~\ref{alg:secure_dp_sgd} amplifies the privacy guarantee of the training process by randomly sampling minibatches from the logically global dataset.  We apply the recently proposed oblivious shuffling protocols~\cite{chida2019efficient, movahedi2015secure, laur2011round}, each of which can securely shuffle the logically global dataset while keeping the new permutation of data samples invisible to parties, to implement the random sample operation. With these oblivious shuffling protocols, we can securely sample minibatches to meet the requirement of DPSGD.}
\end{quote}



]


\twocolumn[

\noindent2-d) and 3-e), in Section~\ref{subsec:secure_DPSGD}, we clarify the phase of decryption as follows:
\begin{quote}
    

\noindent\textcolor{blue}{Note that the model parameters are kept in the secret shared form through the whole secure DPSGD process.}
\end{quote}
\noindent4-f), in Section~\ref{pre:smpc}, we clarify the equality of parties in MPL as follows:

\begin{quote}

\noindent \textcolor{blue}{Note that in our computation process,  all parties are usually equal to each other. This feature is different from federated learning~\cite{yang2019federated}, where there is usually a central server among parties.}
\end{quote}
\noindent4-g), in Section~\ref{pre:smpc}, we modify the ``Encryption and Decryption'' to ``Secret Sharing and Reconstruction'' as follows:

\begin{quote}

\noindent\textcolor{blue}{\textbf{Secret Sharing and Reconstruction.} For additive secret sharing~\cite{ref_gmw}, given a secret $x$, we first generate $m-1$ random number $\share{x}_1, \share{x}_2, \cdots, \share{x}_{m-1}$, and let $\share{x}_m = x  - \sum_{i=1}^{m-1}\share{x}_i$. $P_i$ holds $\share{x}_i$. To reconstruct $x$, all parties exchange $\share{x}_i$ and add them together to obtain $x$. For Shamir's secret sharing~\cite{ref_bgw}, given a secret $x$, we first generate a polynomial $f(y) = a_0 + a_1y+a_2y^2+...+a_ty^t$, where $a_0=x, a_1,\cdots,a_t $ are random coefficients, and $t+1$ is the least number of parties to reconstruct the secret; then we construct $m$ points out of it with indexes $1\leq i \leq m$. These $f(i)$ (i.e. $\share{x}_i$) are exactly the shares of $x$. To reconstruct $x$, all or some of all parties exchange $\share{x}_i$ and reconstruct the polynomial $f(y)$ with the Lagrange interpolation to obtain $x$.}
\end{quote}

\vspace{0.1in}
\textbf{Comment:} \textit{ Moreover, this approach seems to accept only few number of participants that have to be available at each round (to encrypt and decrypt). Could you please give a realistic scenario where this is the case?}

 \vspace{0.05in}  
\textbf{Response:}  Thanks for the insightful comment. We describe one application scenario of our proposed secure DPSGD protocol and its optimization implementations in Section~\ref{related_work}.
]

==> tex/storage.tex <==
\vspace{-2mm}
\section{Missing Proofs}\label{Missing Proof}
\noindent \textbf{Proof of Lemma~\ref{parallel_composition}.} For $n$ mechanisms $M_1, M_2, \cdots, M_n$  whose inputs are disjoint datasets $D_1, D_2, \cdots, D_n$, if $M_i$ satisfies ($\epsilon_i, \delta_i$)-differential privacy, the combination of them satisfies ($\epsilon$, $\delta$)-differential privacy  for the dataset  $D = D_1 \cup D_2 \cup \cdots \cup D_n$ with $\epsilon = Max(\epsilon_1, \epsilon_2, \cdots, \epsilon_n)$, $\delta = Max(\delta_1, \delta_2, \cdots, \delta_n)$. 
\begin{proof}
We first redefine ($\epsilon, \delta$)-differential privacy in a new form based on the definition of ~\cite{parallel_composition}.
\begin{myDef}\label{new_def_dp}
For two datasets $D$ and $D'$, we say a random mechanism M that outputs \begin{math}r \in R^p\end{math} satisfies ($\epsilon, \delta$)-differential privacy if for any subset $S \subseteq  R^p$,
$Pr(M(D) \in S) \leq e^{\epsilon * |D\oplus D'|} \cdot Pr (M(D') \in S) +  \delta * |D\oplus D'|$
\end{myDef}
\noindent where $D\oplus D'$ is the symmetric difference between $D$ and $D'$. 
\noindent Then for $D_1, D_2, \cdots, D_n$ and $D'_1, D'_2, \cdots, D'_n$, let $M$ be the combination of $M_1, M_2, \cdots, M_n$, thus the probability that $M$ outputs $r$ is
    $Pr(M(D) = r) = \prod_{i = 1}^n Pr(M_i(D_i) = r_i) $

Then applying Definition~\ref{new_def_dp},
\begin{small}
\begin{align*}
&\quad\prod_{i = 1}^n Pr(M_i(D_i) = r_i) \\
&\leq \prod_{i = 1}^n (e^{\epsilon_i * |D_i\oplus D'_i|} Pr(M_i(D'_i) = r_i) + \delta_i * |D_i\oplus D'_i|)
\end{align*}
\end{small}
As $D$ and $D'$ are neighboring datasets (i.e., we can obtain $D'$ by deleting or adding one data sample of $D$), there is only one $|D_i\oplus D'_{i}|$ larger than 0, which is equal to $|D\oplus D'|$, and others equal to 0. Without loss of generality, we assume $|D_k\oplus D'_{k}| > 0$. Therefore, 

\begin{small}
\begin{align*}
&\quad \prod_{i = 1}^n (e^{\epsilon_i * |D_i\oplus D'_i|} Pr(M_i(D'_i) = r_i) + \delta_i * |D_i\oplus D'_i|)\\
& = (\prod_{i = 1, i \neq k}^n Pr(M_i(D'_i) = r_i)) *(e^{\epsilon_k * |D_k\oplus D'_k|}Pr(M_k(D'_k) = r_k)\\
&\quad + \delta_k *|D_k\oplus D'_k|)\\
% & \leq (\prod_{i = 1, i \neq k}^n Pr(M_i(D'_i) = r_i)) \\
% &\quad * (e^{Max(\epsilon_1, \epsilon_2, \cdots, \epsilon_n)* |D_k\oplus D'_k|} *Pr(M_k(D'_k) = r_k)\\
% &\quad + Max(\delta_1, \delta_2, \cdots, \delta_n) * |D_k\oplus D'_k|)\\
&\leq e^{Max(\epsilon_1, \epsilon_2, \cdots, \epsilon_n) * |D_k\oplus D'_k|}\prod_{i = 1}^n Pr(M_i(D'_i) = r_i)\\
&\quad + (\prod_{i = 1, i \neq k}^n Pr(M_i(D'_i) = r_i)) * Max(\delta_1, \delta_2, \cdots, \delta_n) * |D_k\oplus D'_k|\\
&\leq  e^{Max(\epsilon_1, \epsilon_2, \cdots, \epsilon_n) * |D\oplus D'|}\prod_{i = 1}^n Pr(M_i(D'_i) = r_i)\\
&\quad+ Max(\delta_1, \delta_2, \cdots, \delta_n)* |D\oplus D'|
\end{align*}
\end{small}
It completes proof.
\end{proof}


\noindent \textbf{Proof of Lemma~\ref{lemma:error_bound}.} For any $x \in [0.5, 1),  (0.8277x^2-2.046x+2.223-0.0048) -\frac{1}{\sqrt{x}} < 0$.

\begin{proof}
Let $f(x) = (0.8277x^2-2.046x+2.223-0.0048) -\frac{1}{\sqrt{x}}$. As function $f$ is differentiable on interval $[0.5, 1)$, we can get its first-order derivative function as  $f'(x) = 1.6554x-2.046 + \frac{1}{2\sqrt{x^{3}}} $ and second-order derivative function as $f''(x) = 1.6554 - \frac{3}{4\sqrt{x^{5}}}$. Because $f''(x)$ is monotonically increasing on $[0.5, 1)$ and has one zero point $x_0 = 0.7286$, $f'(x)$ is monotonically decreasing on $[0.5, 0.7286)$ and monotonically increasing on $[0.7286, 1)$. Then as $f'(0.7286) = -0.0359 < 0$ and $f'(x)$ is larger than 0 on two endpoints $0.5$ and $1$, $f'(x)$ has two zero points on $[0.5, 1)$: $x_1 = 0.6257$ and $x_2 = 0.8517$. Therefore, $f(x)$ is monotonically increasing on $[0.5, 0.6257)$, monotonically decreasing on $[0.6257, 0.8517)$, and monotonically increasing on $[0.8517, 1)$. Finally, for any $x \in [0.5, 1)$, $f(x) < \max\{f(0.6257), f(1)\} = -0.0001 < 0$. 
\end{proof}


\noindent \textbf{Proof of Theorem~\ref{theo:secure_dp_sgd}.}   For any $\epsilon \leq 2\log(1/\delta)$ and $\delta \in (0, 1)$,  Protocol~\ref{alg:secure_dp_sgd} satisfies ($\epsilon, \delta$)-differential privacy.

\begin{proof}
We first introduce a novel differential privacy concept, namely R\'enyi differential privacy (RDP), to tightly analyze the privacy budget of DPSGD in a simple way.

\begin{myDef}
\textbf{($\lambda,\gamma$)-R\'enyi Differential Privacy~\cite{renyi}.}  For a random mechanism M whose input is \begin{math}D\end{math} and output \begin{math}r \in R^p\end{math}, we say M satisfies  \begin{math}(\lambda,\gamma)\end{math}-RDP if for any two neighboring datasets $D, D'$, it holds that,
\begin{center}
\scalebox{0.9}{
    \begin{math}
    D_{\lambda}(M(D)\|M(D')) \leq \gamma
    \end{math}
}
\end{center}
\end{myDef}
\noindent where $D_{\lambda}(M(D)\|M(D'))$ is $\lambda$-R\'enyi divergence between the distributions of $M(D)$ and $M(D')$. Then we introduce privacy properties of RDP~\cite{renyi}.

\begin{lemma}\label{gaussian_rdp}
 Let $C = max_{D\sim D'}\left\|f(D) - f(D') \right\|$ be the $L_2$ sensitivity of $f$, then $M = f(D) + b$ satisfies ($\lambda, \frac{\lambda C^2}{2\sigma^{2}}$)-RDP, where $b \sim \mathcal{N}(0, \sigma^2I_{p\times p})$. 
\end{lemma}

\begin{lemma}\label{composition_rdp}
For n mechanisms $M_1, M_2, \cdots, M_n$ that access the same dataset D, if each $M_i$ satisfies ($\lambda$, $\gamma_i$)-RDP, the combination of their outputs satisfies ($\lambda$, $\gamma$)-RDP with $\gamma =\gamma_1 + \gamma_2 + \cdots + \gamma_n$.
\end{lemma}

\begin{lemma}\label{conversion_rdp}
If a randomized mechanism M satisfies ($\lambda, \gamma$)-RDP, then M satisfies ($\gamma+ \frac{log(\frac{1}{\delta})}{\lambda - 1}, \delta$)-differential privacy for any $\delta \in (0, 1)$.
\end{lemma}


According to Lemma~\ref{lemma:error_bound}, the maximum difference between the approximated $\frac{1}{\sqrt{x'}}$ and true $\frac{1}{\sqrt{x'}}$ is smaller than 0. Thus Protocol~\ref{alg:secure_inversesqrt} can ensure that for each iteration, the $L_2$ sensitivity of Protocol~\ref{alg:secure_dp_sgd} is smaller than $C$. Then each iteration of Protocol~\ref{alg:secure_dp_sgd} satisfies ($\lambda, \frac{\lambda C^{2}}{2\sigma^{2}}$)-RDP because of Lemma~\ref{gaussian_rdp}. According to Lemma~\ref{composition_rdp}, Protocol~\ref{alg:secure_dp_sgd} satisfies ($\lambda,  T\frac{\lambda C^{2}}{2\sigma^{2}}$)-RDP. Finally, \wqruan{according to Lemma~\ref{conversion_rdp}}, in order to ensure ($\epsilon, \delta$)-differential privacy, we need to ensure that
\begin{center}
    \begin{math}
    \frac{TC^{2}\lambda}{2\sigma^{2}} + \frac{\log(\frac{1}{\delta})}{\lambda - 1} \leq \epsilon
    \end{math}
\end{center}
\noindent We set $\lambda = 1 + \frac{2\log(\frac{1}{\delta})}{\epsilon}$, thus we need to ensure that
\begin{center}
    \begin{math}
    \sigma^{2} \geq \frac{TC^{2}(\epsilon+2\log(\frac{1}{\delta}))}{\epsilon^{2}} 
    % 
    \end{math}
\end{center}
\noindent Meanwhile, as we set in Protocol~\ref{alg:secure_dp_sgd}
\begin{center}
    \begin{math}
    \sigma^2 \geq \frac{TC^{2}(4\log(\frac{1}{\delta}))}{\epsilon^{2}} \geq \frac{TC^{2}(\epsilon+2\log(\frac{1}{\delta}))}{\epsilon^{2}} 
    \end{math}
\end{center}
Therefore, Protocol~\ref{alg:secure_dp_sgd} satisfies ($\epsilon, \delta$)-differential privacy.
\end{proof}


\noindent\textbf{Proof of Theorem~\ref{theo:model_initialization}.} Protocol~\ref{alg:global_model_initialization} satisfies ($\epsilon_1, \delta_1$)-differential privacy.
\begin{proof}
 Each local dataset $D_i$ held by $P_i$ can be viewed as a subset of the logically global dataset. Meanwhile, as different parties hold different data, their local datasets are disjoint. In addition, the aggregation methods are data-independent. According to the post-process immunity property of differential privacy, the aggregation has no impact on the privacy guarantee. Therefore, we only need to consider the privacy guarantee of local model training. 
 As all parties privately train their models with privacy parameters ($\epsilon_1, \delta_1$), we can obtain the privacy guarantee of Protocol~\ref{alg:global_model_initialization} by directly applying Lemma~\ref{parallel_composition}. 
\end{proof}


\section{Experiment Settings}\label{parameter setting}


\begin{table}
\centering
\caption{Hyperparameters setting of local model training.}
\label{tab:local_model_paramters}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Datasets} & \textbf{$\epsilon$} & \textbf{$\delta$} & \textbf{Clip bound} & \textbf{\#Epoch} & \textbf{Batch size} & \textbf{LR} \\ \hline
MNIST    & 0.25                        &      $2\times10^{-7}$                 &     1           &    3       &        128    &          0.1     \\ \hline
CIFAR-10 &    0.25                     &    $1.7\times10^{-7}$                     &   1          &    1       &    128        &     0.1          \\ \hline
IMDb     & 0.25                        &      $4\times10^{-7}$                   &       1         &    3       &    128       &     0.1          \\ \hline
\end{tabular}}
\end{table}


\begin{table}
\centering

\caption{Potential hyperparameters involved in the grid search procedure of baselines training.}
\label{tab:baseline_grid_search_paramters}
\scalebox{0.85}{
\begin{tabular}{|c|c|}
\hline
\textbf{Hyperparameter}          &   \textbf{Potential values}                            \\  \hline
Clipping bound          &   1, 2, 5                                     \\  \hline
Batch size              &   64, 128, 256, 512                               \\  \hline
Learning rate schedule  &   Constant (lr=0.1), OneCycleLR (max\_lr=0.1) \\  \hline

\end{tabular}}
\end{table}

\begin{table}
\centering

\caption{Hyperparameters setting of baseline model training.}
\label{tab:baseline_paramters}
\scalebox{0.9}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Datasets} & \textbf{Clipping bound} & \textbf{Batch size} & \textbf{LR} \\ \hline
MNIST    &     1          &    128     & Constant (lr=0.1)     \\ \hline
CIFAR-10 &     1          &    512     & OneCycleLR (max\_lr=0.1)  \\ \hline
IMDb     &     2          &    64      & OneCycleLR (max\_lr=0.1)   \\ \hline
\end{tabular}}
\end{table}


In this section, we show the hyperparameters setting of experiments. The hyperparamters of local model training are shown in Table~\ref{tab:local_model_paramters}.  The potential hyperparameters involved in the grip search procedure are shown in Table~\ref{tab:baseline_grid_search_paramters}.  We also show the parameters found by the grid search procedure in Table~\ref{tab:baseline_paramters}. Note that we run baseline training process of CIFAR-10, MNIST, and IMDb for 80, 20, 20 epochs, respectively.




\section{Aggregation Methods}
\label{sec:aggregation}
In this section, we introduce two aggregation methods of Section~\ref{subsec:initialization}. We show the details of the average aggregation method and choosing the most accurate local model method in Protocol~\ref{alg:average_aggregation} and Protocol~\ref{alg:maximum_aggregation}, respectively. We then analyze the complexity of each aggregation method as follows.

\begin{algorithm}
\small
\caption{Average Aggregation }
\label{alg:average_aggregation}
\begin{algorithmic}[1]
\REQUIRE  Each party $P_i$ holds a local model $\theta^{l}_i$.
\ENSURE Each party $P_i$ obtains the share of the average of local models $\share{\theta_{a}}_i$;
\STATE $P_i$ sends the share of its local model $\share{\theta^{l}_{i}}_{j \neq i}$ to other parties;
\STATE $P_i$ compute $\share{\theta_{a}}_i = \sum_{j = 1}^{m} \share{\theta^{l}_j}_{i} / m$;
\STATE $P_i$ obtains $\share{\theta_{a}}_i$ as the share of the average of local models;
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\small
\caption{Most Accurate Local Model }
\label{alg:maximum_aggregation}
\begin{algorithmic}[1]
\REQUIRE Each party $P_i$ holds a local model $\theta^{l}_i$.
\ENSURE Each party $P_i$ obtains the share of the most accurate local model $\share{\theta_{m}}_i$;
\STATE $P_i$ sends the share of its local model $\share{\theta^{l}_{i}}_{j \neq i}$ to other parties and initializes $Accuracy_m$ as 0;
\FOR{Each $\theta^{l}_i \in \{\theta^{l}_1, \theta^{l}_2, \cdots, \theta^{l}_m \}$}
\STATE All parties collaboratively test the accuracy of $\theta^{l}_i$ as $Accuracy_{i}$;
\IF{$Accuracy_{i} \geq$  $Accuracy_m$}
\STATE $\share{\theta_{m}} = \share{\theta^{l}_i}$;
\STATE $Accuracy_m = Accuracy_{i}$;
\ENDIF
\ENDFOR
\STATE $P_i$ obtains $\share{\theta_{m}}_i$ as the share of the most accurate local model;
\end{algorithmic}
\end{algorithm}

\noindent\textbf{Complexity of Protocol~\ref{alg:global_model_initialization}.}
We first analyze the complexity of Protocol~\ref{alg:average_aggregation} and Protocol~\ref{alg:maximum_aggregation}. Protocol~\ref{alg:average_aggregation} only includes a constant division computation and needs to perform one $\mathsf{Trunc}$ computation. Hence, Protocol~\ref{alg:average_aggregation} needs 2 communication rounds and $O(pk)$ bits communication. For Protocol~\ref{alg:maximum_aggregation}, the main overhead is from the accuracy test of each local model. Assuming the size of the testing dataset is $n_t$, the communication round complexity of Protocol~\ref{alg:maximum_aggregation} is $O(m)$ and the communication overhead is $O(mn_tpk)$, where the constant depends on the complexity of the trained model. 




We then analyze the complexity of Protocol~\ref{alg:global_model_initialization} introduced in Section~\ref{subsec:initialization}. Besides the invocations of Protocol~\ref{alg:average_aggregation} and Protocol~\ref{alg:maximum_aggregation}, Protocol~\ref{alg:global_model_initialization} test the accuracy of two candidate models. Thus its communication round complexity is $O(m)$ and communication overhead is $O((mn_t+1)pk)$.





\section{Missing experimental results of Section~\ref{subsec:effectiveness_MPL}}~\label{missing_res_MPL}

\begin{table}
\centering
\caption{Accuracy (in \%) comparison of locally trained  models and globally trained models for MNIST. We report the average results of five runs and show standard deviations in brackets. As \tfencrypted only supports the 3-party scenario, we show the 3-party result of it.  }
\label{tab:effectiveness_MPL_MNIST}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\#Party}          & \textbf{$\epsilon$} & \textbf{Local party} & \textbf{\tfencrypted} & \textbf{\queqiao} \\ \hline
\multirow{3}{*}{3-party}  & 0.25                & $87.23\; (\pm 0.34)$ & $89.36\; (\pm 0.25)$                 & $89.50\; (\pm 0.22)$             \\ \cline{2-5} 
                          & 1                   & $93.56\; (\pm 0.22)$ & $95.03\; (\pm 0.11)$                 & $94.04\; (\pm 0.21)$             \\ \cline{2-5} 
                          & 2                   & $94.25\; (\pm 0.15)$ & $95.14\; (\pm 0.09)$                 & $94.90\; (\pm 0.14)$             \\ \hline
\multirow{3}{*}{5-party}  & 0.25                & $86.92\; (\pm 0.39)$ & -                                    & $88.18\; (\pm 0.21)$             \\ \cline{2-5} 
                          & 1                   & $92.33\; (\pm 0.29)$ & -                                    & $93.99\; (\pm 0.09)$             \\ \cline{2-5} 
                          & 2                   & $93.92\; (\pm 0.24)$ & -                                    & $95.13\; (\pm 0.19)$             \\ \hline
\multirow{3}{*}{10-party} & 0.25                & $79.23\; (\pm 2.23)$ & -                                    & $85.60\; (\pm 0.58)$             \\ \cline{2-5} 
                          & 1                   & $89.25\; (\pm 0.37)$ & -                                    & $94.32\; (\pm 0.31)$             \\ \cline{2-5} 
                          & 2                   & $92.96\; (\pm 0.21)$ & -                                    & $95.35\; (\pm 0.15)$             \\ \hline
\end{tabular}}
\end{table}

\begin{table}[ht]
\centering
\caption{Accuracy (in \%) comparison of locally trained  models and globally trained models for IMDb. We report the average results of five runs and show standard deviations in brackets. As \tfencrypted only supports the 3-party scenario, we show the 3-party result of it. }
\label{tab:effectiveness_MPL_IMDb}
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\#Party}          & \textbf{$\epsilon$} & \textbf{Local party} & \textbf{\tfencrypted} & \textbf{\queqiao} \\ \hline
\multirow{3}{*}{3-party}  & 0.25                & $79.48\; (\pm 0.72)$ & $80.55\; (\pm 0.49)$                 & $80.20\; (\pm 0.51)$             \\ \cline{2-5} 
                          & 1                   & $83.84\; (\pm 0.32)$ & $84.46\; (\pm 0.67)$                 & $84.49\; (\pm 0.28)$             \\ \cline{2-5} 
                          & 2                   & $84.08\; (\pm 0.19)$ & $84.70\; (\pm 0.44)$                 & $84.35\; (\pm 0.17)$             \\ \hline
\multirow{3}{*}{5-party}  & 0.25                & $77.2\; (\pm 1.01)$  & -                                    & $77.46\; (\pm 0.82)$             \\ \cline{2-5} 
                          & 1                   & $80.33\; (\pm 0.26)$ & -                                    & $84.01\; (\pm 0.15)$             \\ \cline{2-5} 
                          & 2                   & $80.69\; (\pm 0.21)$ & -                                    & $84.59\; (\pm 0.37)$             \\ \hline
\multirow{3}{*}{10-party} & 0.25                & $72.00\; (\pm 1.81)$ & -                                    & $75.48\; (\pm 1.03)$             \\ \cline{2-5} 
                          & 1                   & $77.84\; (\pm 1.30)$ & -                                    & $84.64\; (\pm 0.13)$             \\ \cline{2-5} 
                          & 2                   & $78.22\; (\pm 0.69)$ & -                                    & $84.56\; (\pm 0.31)$             \\ \hline
\end{tabular}}
\end{table}
In this section, we show the accuracy comparison results of locally trained models and global models for MNIST and IMDb. The results are shown in Table~\ref{tab:effectiveness_MPL_MNIST} and Table~\ref{tab:effectiveness_MPL_IMDb}. Like the results of CIFAR-10, the accuracy of the global models is higher than locally trained models in all scenarios. Meanwhile, the accuracy gaps between locally trained models and global models also become larger as the number of parties increases. These results further verify the effectiveness of training models on the logically global datasets that are composed of local datasets through MPL.


Instead of training an end-to-end neural network model, \wqruan{we let} each party first applies data-independent feature extractors, including foundation models~\cite{foundation_model} (e.g. BERT~\cite{BERT}) and feature extraction rules, to extract features of input datasets locally. Consequently, all parties collaboratively train shallow models (e.g. linear models or neural network models with a few layers) on extracted features. In this way, parties only need to perform secure computation and add noise in the shallow model training process. As a result, the accuracy loss and communication overhead can be significantly reduced.
